A General Pipeline for Glomerulus Whole-Slide Image Segmentation

Whole-slide images (WSI) glomerulus segmentation is essential for accurately diagnosing kidney diseases. In this work, we propose a general and practical pipeline for glomerulus segmentation that effectively enhances both patch-level and WSI-level segmentation tasks. Our approach leverages stitching on overlapping patches, increasing the detection coverage, especially when glomeruli are located near patch image borders. In addition, we conduct comprehensive evaluations from different segmentation models across two large and diverse datasets with over 30K glomerulus annotations. Experimental results demonstrate that models using our pipeline outperform the previous state-of-the-art method, achieving superior results across both datasets and setting a new benchmark for glomerulus segmentation in WSIs. The code and pre-trained models are available at https://github.com/huuquan1994/wsi_glomerulus_seg.

==> conflicts_of_interest.tex <==
No funding was received for conducting this study. 
The authors have no relevant financial or non-financial interests to disclose.

==> ethical_standards.tex <==
This research study was conducted retrospectively using animal subject data made available in open access by \cite{tang2024holohisto} and \cite{stritt2020orbit}. 
Ethical approval was not required as confirmed by the license attached with the open access data. 
